Singular Value Decomposition in Sobolev Spaces: Part I

A well known result from functional analysis states that any compact operator between Hilbert spaces admits a singular value decomposition (SVD). This decomposition is a powerful tool that is the workhorse of many methods both in mathematics and applied fields. A prominent application in recent years is the approximation of high-dimensional functions in a low-rank format. This is based on the fact that, under certain conditions, a tensor can be identified with a compact operator and SVD applies to the latter. One key assumption for this application is that the tensor product norm is not weaker than the injective norm. This assumption is not fulfilled in Sobolev spaces, which are widely used in the theory and numerics of partial differential equations. Our goal is the analysis of the SVD in Sobolev spaces. This work consists of two parts. In this manuscript (part I), we address low-rank approximations and minimal subspaces in H1. We analyze the H1-error of the SVD performed in the ambient L2-space. In part II, we will address variants of the SVD in norms stronger than the L2-norm. We will provide a few numerical examples that support our theoretical findings.

==> Sections/conclusion.tex <==
\section{Conclusion}\label{sec:concl}
We proposed and analyzed several variants of
low-rank approximations of functions in Sobolev spaces.
Sets of functions with bounded Tucker (multi-linear) rank
in Sobolev spaces are weakly closed. Sobolev functions can
be shown to be in the tensor product of their minimal subspaces under certain
conditions, such as additional regularity. However, we do not believe that
this holds in general.

The $L^2$-SVD preserves regularity of the decomposed functions and, under
certain conditions, we can quantify the $H^1$ error in terms of the rescaled
singular values. We show that the singular values of different SVDs are closely
related. Lower and upper bounds are obtained by simple scalings.

We also analyze $H^1$ minimal subspaces. The SVD in $H^{(1,0)}$ does not
preserve regularity and $H^1$ bounds require additional smoothness.
The resulting bounds are worse than that of the $L^2$-SVD. Similar
bounds apply to spaces of lower order mixed smoothness for $d>2$.
This indicates the $L^2$-SVD performs better for low-rank
approximations than variants of SVDs involving Sobolev spaces.

Numerical experiments are consistent with the analytical findings.
Differences
between minimal subspaces w.r.t.\ to different norms arise only when
considering functions in Sobolev spaces that are not in the
algebraic tensor spaces.
For
constructing low-rank approximations of numerical solutions, the
different types of minimal subspaces do not add information. However,
the singular values of $H^{(1,0)}$-, $H^{(0,1)}$-SVDs
are better suited to estimate the
$H^1$ error and, for numerical purposes, it seems the best recipe are
low-rank approximations built from $L^2$-SVDs but with $H^{(1,0)}$,
$H^{(0,1)}$ singular
values for $H^1$-error control.

Finally, we briefly mentioned alternatives. Exponential sums are a well known
technique already utilized in previous works. On the other hand, if one
pursues the viewpoint of Sobolev spaces being intersection spaces, a natural
approach would be to consider direct sum spaces. We briefly introduced this
viewpoint.

There are a few immediate open questions that arise in conclusion of this work.
It would be interesting to consider how the above analysis extends
to hierarchical tensor formats. Numerical experiments for high-dimensional
problems with a fine or adaptive discretization
should shed more light on the performance of SVD in Sobolev spaces.

